NLP-based Automated Compliance Checking of Data Processing Agreements against GDPR

Processing personal data is regulated in Europe by the General Data Protection Regulation (GDPR) through data processing agreements (DPAs). Checking the compliance of DPAs contributes to the compliance verification of software systems as DPAs are an important source of requirements for software development involving the processing of personal data. However, manually checking whether a given DPA complies with GDPR is challenging as it requires significant time and effort for understanding and identifying DPA-relevant compliance requirements in GDPR and then verifying these requirements in the DPA. In this paper, we propose an automated solution to check the compliance of a given DPA against GDPR. In close interaction with legal experts, we first built two artifacts: (i) the "shall" requirements extracted from the GDPR provisions relevant to DPA compliance and (ii) a glossary table defining the legal concepts in the requirements. Then, we developed an automated solution that leverages natural language processing (NLP) technologies to check the compliance of a given DPA against these "shall" requirements. Specifically, our approach automatically generates phrasal-level representations for the textual content of the DPA and compares it against predefined representations of the "shall" requirements. Over a dataset of 30 actual DPAs, the approach correctly finds 618 out of 750 genuine violations while raising 76 false violations, and further correctly identifies 524 satisfied requirements. The approach has thus an average precision of 89.1%, a recall of 82.4%, and an accuracy of 84.6%. Compared to a baseline that relies on off-the-shelf NLP tools, our approach provides an average accuracy gain of ~20 percentage points. The accuracy of our approach can be improved to ~94% with limited manual verification effort.

==> acknowledgement.tex <==
\sectopic{Acknowledgment}
This paper was supported by Linklaters, Luxembourg's National Research Fund (FNR) under grant BRIDGES/19/IS/13759068/ARTAGO, and NSERC of Canada under the Discovery, Discovery Accelerator and CRC programs. The authors would like to specially thank Katrien Baetens, Sylvie Forastier, Peter Goes and Catherine Freichel from Linklaters LLP for enriching this work through their expertise. 

==> all-requirements-table.tex <==

\begin{table*}[ht!]
\caption{DPA Compliance Requirements in GDPR.}
     \begin{subtable}{\linewidth}
	  \caption{Processor's Obligations}
	  \begin{threeparttable}[t]
	    \begin{tabularx}{\columnwidth}{@{} p{3em} @{\hskip 0.5em} p{7em} @{\hskip 0.5em} X @{}} 
	  \toprule
      \textbf{PO1} & \textit{Art.~28(2)} & The processor shall not engage a sub-processor without a prior specific or general written authorization of the controller. \\ 
      \midrule
      \textbf{PO2} & \textit{Art.~28(2)} & In case of general written authorization, the processor shall inform the controller of any intended changes concerning the addition or replacement of sub-processors. \\
      \midrule
      \textbf{PO3} & \textit{Art.~28(3)(a)} & The processor shall process personal data only on documented instructions from the controller.\\
      \midrule
      \textbf{PO4} & \textit{Art.~28(3)(a)} & If the processor requires by Union or Member State law to process personal data without instructions and law does not prohibit informing the controller on grounds of public interest, the processor shall inform the controller of that legal requirement before processing. \\
      \midrule
      \textbf{PO5} & \textit{Art.~28(3)(b)} & The processor shall ensure that persons authorized to process personal data have committed themselves to confidentiality or are under an appropriate statutory obligation of confidentiality.\\
      \midrule
      \textbf{PO6} & \textit{Art.~28(3)(c)} & The processor shall take all measures required pursuant to Article 32 or to ensure the security of processing.  \\ 
      \midrule
      \textbf{PO7} & \textit{Art.~28(3)(e)} & The processor shall assist the controller in fulfilling its obligation to respond to requests for exercising the data subject's rights. \\ 
      \midrule
      \textbf{PO8} & \textit{Art.~28(3)(f),} \par \textit{Art.~32} & The processor shall assist the controller in ensuring the security of processing.  \\ 
      \midrule
      \textbf{PO9} & \textit{Art.~28(3)(f),} \par \textit{Art.~36} & The processor shall assist the controller in consulting the supervisory authorities prior to processing where the processing would result in a high risk in the absence of measures taken by the controller to mitigate the risk. \\ 
      \midrule
      \textbf{PO10} & \textit{Art.~28(3)(f),} \par \textit{Art.~33} & The processor shall assist the controller in notifying a personal data breach to the supervisory authority.\\ 
      \midrule
      \textbf{PO11} & \textit{Art.~28(3)(f),} \par \textit{Art.~34} & The processor shall assist the controller in communicating a personal data breach to the data subject.  \\ 
      \midrule
      \textbf{PO12} & \textit{Art.~28(3)(f),} \par \textit{Art.~35} & The processor shall assist the controller in ensuring compliance with the obligations pursuant to data protection impact assessment (DPIA).  \\ 
      \midrule
      \textbf{PO13} & \textit{Art.~28(3)(g)} & The processor shall return or delete all personal data to the controller after the end of the provision of services relating to processing.\\ 
      \midrule
      \textbf{PO14} & \textit{Art.~28(3)(h)} & The processor shall immediately inform the controller if an instruction infringes the GDPR or other data protection provisions. \\
        \midrule
      \textbf{PO15} & \textit{Art.~28(3)(h)} & The processor shall make available to the controller information necessary to demonstrate compliance with the obligations Article 28 in GDPR. \\
      \midrule
      \textbf{PO16} & \textit{Art.~28(3)(h)} & The processor shall allow for and contribute to audits, including inspections, conducted by the controller or another auditor mandated by the controller. \\ 
      \midrule
      \textbf{PO17} & \textit{Art.~28(4)} & The processor shall impose the same obligations on the engaged sub-processors by way of contract or other legal act under Union or Member State law.\\
      \midrule
      \textbf{PO18} & \textit{Art.~28(4)} & The processor shall remain fully liable to the controller for the performance of sub-processor's obligations.  \\
        \midrule
    \textbf{PO19} & \textit{Art.~32(2)} & When assessing the level of security, the processor shall take into account the risk of accidental or unlawful destruction, loss, alternation, unauthorized disclosure of or access to the personal data transmitted, stored or processed.  \\
    \midrule
    PO20 & \textit{Art.~28(3)(a)} & The processor shall not transfer personal data to a third country or international organization without  a prior specific or general authorization of the controller.  \\
   \midrule
   PO21 & \textit{Art.~28(5)} & The processor can demonstrate guarantees to Article 28 (1--4) through adherence to an approved codes of conduct or an approved certification mechanism.  \\
   \midrule
   PO22 & \textit{Art.~32(1)} & The processor shall implement appropriate technical and organisational measures to ensure a level of security appropriate to the risk of varying likelihood and severity for the rights and freedoms of natural persons. \\
   \midrule
   PO23 & \textit{Art.~32(4)} & The processor shall ensure that any natural person acting under its authority who has access to personal data only process them on instructions from the controller. \\
   \midrule
   PO24 & \textit{Art.~33(2)} & The processor shall notify the controller without undue delay after becoming aware of a personal data breach. \\
   \midrule
   PO25 & \textit{Art.~82(2)} & A processor shall be liable for the damage caused by processing only where it has not complied with GDPR obligations specifically directed to processors or where it has acted outside or contrary to lawful instructions of the controller. \\ 
   \bottomrule
	  \end{tabularx}
	\begin{tablenotes}
    \item[1] GDPR-related articles.
    \end{tablenotes}
    \end{threeparttable}
	  \label{tab:table_d}
	  \end{subtable} 
\end{table*}

\begin{table*}[ht!]
\ContinuedFloat
  \caption{DPA-related Requirements in GDPR (continued).}  
 \label{tab:requirements}
  \centering
  \begin{subtable}{\linewidth}
    \caption{Metadata}
    \begin{threeparttable}[t]
    \begin{tabularx}{\columnwidth}{@{} p{3em} @{\hskip 0.5em} p{7em} @{\hskip 0.5em} X @{}} 
    \toprule
        \textbf{ID} & \textbf{Reference}\tnote{1} & \textbf{Requirement} \\
    \midrule
        \textbf{MD1} & \textit{Legal Experts} & The DPA shall contain at least one controller's identity and contact details.\\
    \midrule
       \textbf{MD2} & \textit{Legal Experts} & The DPA shall contain at least one processor's identity and contact details.\\
    \midrule
       \textbf{MD3} & \textit{Art.~28(3)} & The DPA shall contain the duration of the processing.\\
    \midrule
       \textbf{MD4} & \textit{Art.~28(3)} & The DPA shall contain the nature and purpose of the processing.\\  
    \midrule
       \textbf{MD5} & \textit{Art.~28(3)} & The DPA shall contain the types of personal data.\\ 
    \midrule
       \textbf{MD6} & \textit{Art.~28(3)} & The DPA shall contain the categories of data subjects.\\
    \midrule
        MD7 & \textit{Art.~32(1)} & The  organizational and technical measures to ensure a level of security can include: (a) pseudonymisation and encryption of personal data, (b) ensure confidentiality, integrity, availability and resilience of processing systems and services, (c) restore the availability and access to personal data in a timely manner in the event of a physical or technical incident, and (d) regularly testing, assessing and evaluating the effectiveness of technical and organisational measures for ensuring the security of the processing. \\  
    \midrule
       MD8 & \textit{Art.~33(3)} & The notification of personal data breach shall at least include (a) the nature of personal data breach; (b) the name and contact details of the data protection officer; (c) the consequences of the breach; (d) the measures taken or proposed to mitigate its effects.\\
       \midrule
       MD9 & \textit{Art.~35(7)} & The DPIA shall at least include (a) a systematic description of the envisaged processing operations and the purposes of the processing, (b) an assessment of the necessity and proportionality of the processing operations in relation to the purposes, (c) an assessment of the risks to the rights and freedoms of data subjects, and (d) the measures envisaged to address the risks.\\
    \midrule
      \end{tabularx}
     \end{threeparttable}
      \label{tab:table_a}
    \end{subtable}
    
    \begin{subtable}{\linewidth}
    \vspace*{1em}
    \caption{Controller's Obligations}
      \begin{threeparttable}[t]
        \begin{tabularx}{\columnwidth}{@{} p{3em} @{\hskip 0.5em} p{7em} @{\hskip 0.5em} X @{}} 
        \midrule
          CO1 & \textit{Art.~33(1)} & The controller shall, no later than 72 hours after having become aware of personal data breach, notify it to the supervisory authority.\\ 
          \midrule
           CO2 & \textit{Art.~33(5)} & The controller shall document personal data breaches.\\ 
          \midrule
           CO3 & \textit{Art.~34(1)} & In case of high risks, the controller shall communicate the data breach to the data subject without undue delay.\\ 
          \midrule
           CO4 & \textit{Art.~35(1)} & The controller shall carry out a DPIA. \\ 
          \midrule
           CO5 & \textit{Art.~35(2)} & The controller shall seek advice of the DPO when carrying a DPIA.\\ 
          \midrule
           CO6 & \textit{Art.~35(9)} & The controller shall seek the views of data subjects or their representatives on the intended processing.\\ 
          \midrule
           CO7 & \textit{Art.~35(11)} & The controller shall carry out a review to assess if processing is performed in accordance with the data protection impact assessment at least when there is a change of the risk represented by processing operations.\\ 
          \midrule
           CO8 & \textit{Art.~82(2)} & Any controller involved in processing shall be liable for the damage caused by processing which infringes the GDPR.\\ 
        \midrule
        \end{tabularx}
      \begin{tablenotes}
         \item[1] GDPR-related articles.
       \end{tablenotes}
 \end{threeparttable}
    \label{tab:table_b}
 \end{subtable} 
 
 \begin{subtable}{\linewidth}
    \vspace*{1em}
      \caption{Controller's Rights}
      \begin{tabularx}{\columnwidth}{@{} p{3em} @{\hskip 0.5em} p{7em} @{\hskip 0.5em} X @{}} 
        \midrule
           \textbf{CR1} & \textit{Art.~8(2)} & In case of general written authorization, the controller shall have the right to object to changes concerning  the addition or replacement of sub-processors, after having been informed of such intended changes by the processor. \\ 
          \midrule
           CR2 & \textit{Legal Experts} & The controller shall have the right to suspend the processing in certain cases.\\ 
         \midrule
            CR3 & \textit{Legal Experts} & The controller shall have the right to terminate the DPA in certain cases.\\ 
        \midrule
    \end{tabularx}
    \label{tab:table_c}
  \end{subtable} 
\end{table*}

